MOVI: A Model-Free Approach to Dynamic Fleet Management

Modern vehicle fleets, e.g., for ridesharing platforms and taxi companies, can reduce passengers' waiting times by proactively dispatching vehicles to locations where pickup requests are anticipated in the future. Yet it is unclear how to best do this: optimal dispatching requires optimizing over several sources of uncertainty, including vehicles' travel times to their dispatched locations, as well as coordinating between vehicles so that they do not attempt to pick up the same passenger. While prior works have developed models for this uncertainty and used them to optimize dispatch policies, in this work we introduce a model-free approach. Specifically, we propose MOVI, a Deep Q-network (DQN)-based framework that directly learns the optimal vehicle dispatch policy. Since DQNs scale poorly with a large number of possible dispatches, we streamline our DQN training and suppose that each individual vehicle independently learns its own optimal policy, ensuring scalability at the cost of less coordination between vehicles. We then formulate a centralized receding-horizon control (RHC) policy to compare with our DQN policies. To compare these policies, we design and build MOVI as a large-scale realistic simulator based on 15 million taxi trip records that simulates policy-agnostic responses to dispatch decisions. We show that the DQN dispatch policy reduces the number of unserviced requests by 76% compared to without dispatch and 20% compared to the RHC approach, emphasizing the benefits of a model-free approach and suggesting that there is limited value to coordinating vehicle actions. This finding may help to explain the success of ridesharing platforms, for which drivers make individual decisions.

==> experiments_TR.tex <==
For verification and evaluation of the methods described in the previous sections, we create a taxi fleet simulator based on data from New York City~\cite{data}. We implemented both the RHC and DQN frameworks in Python. All machine learning models in this work are modeled and trained using tensorflow \cite{tensor}. In the discussion below, we first discuss our simulation data before outlining the structure of the simulator and our RHC and DQN implementations.

\subsection{Simulation Data}
We base our simulator on NYC Taxi and Limousine Commission taxi trip records from May and June 2016, including the pick-up and drop-off dates/times, pick-up and drop-off locations, and travel distances for each trip~\cite{data}. While each pickup location in this datasets represents where a passenger hailed a taxi on the street, we assume the distribution of passenger demand is similar when the passenger uses a mobile application. We used the dataset in May 2016 for training and June 2016 for testing. We extract trip records in New York City within the area shown in Figure ~\ref{fig:demand}' heat map, which covers more than 95\% of trips in the dataset after removing records with outliers. The colored zones in the figure represent the number of total ride requests in the training data. The weekly demand trends are shown in Figure ~\ref{fig:demand2}, indicating that the demand curves in the training and test dataset exhibit the same periodicity over a week.

\begin{figure}[h]
\centering
\includegraphics[width=0.2\textwidth]{demand}
\caption{Geographical demand distribution}
\label{fig:demand}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{demand2.pdf}
\caption{Weekly demand trend in May and June 2016}
\label{fig:demand2}
\end{figure}


\subsection{Simulator}
In order to train and evaluate our frameworks, we build a simulator of the dispatch center's environment. Figure ~\ref{fig:simulator} shows the architecture of the fleet simulator. The fleet object maintains the states of all vehicles including their current locations, destination locations, estimated times of arrival at destination, and occupancy state. In every time step, all vehicles update their states according to their matching assignments and dispatch orders.

As shown in Algorithm ~\ref{alg:sim}, the simulator first initializes an arbitrary number of vehicles and generates ride requests in each time step based on the real trip records. The agent then computes the actions $a_t$, using either the RHC or DQN framework, and the dispatcher matches appropriate vehicles to requesting customers. When the agent sends a dispatch order to the vehicles, the simulator creates an estimated trajectory to the dispatched location based on the shortest path in the road network graph. We assume that the vehicles move to dispatched locations within the trip time given by our ETA model. If there are no available resources in the customer's region, this ride request is rejected and disappears.

\begin{algorithm}
\small
\caption{Fleet Simulator}\label{alg:sim}
Initialize the fleet state $F_0$\;
\For{$t=0:T_{max}$}
{
Load ride requests within time slot $t$\;
\For{each ride request}{
Select the closest vehicle $n$ to a pickup location\;
Compute dispatch trip time with the ETA model\;
Update $f_t^{(n)}$ according to the assigned ride request\;
}
Output $F_t, W_t$ to an agent\;
Get dispatch orders $a_t$ from an agent\;
\For{$n, d_t^{(n)} \in a_t$}{
Search the shortest path from the $n$-th vehicle location to dispatch location $d_t^{(n)}$\;
Compute dispatch trip time with the ETA model\;
Generate the future trajectory and assign it to the $n$-th vehicle\;
}
Update the fleet state $F_{t+1}$\;
}
\end{algorithm}

The general framework of the dispatch system is the same for both RHC and DQN. We discretize the city into $212 \times 219$ grid regions whose area is around $150 \times 150$ m$^2$. In each time step, the dispatcher selects idle vehicles $\mathcal{I}_t$ from available vehicles, which have not yet received dispatch orders since dropping off passengers the last time or which has not assigned any ride requests last 15 minutes. These preprocessed real-time data are then fed into the dispatcher. In the discussion below, we detail each module except for the agent, which is discussed in Section~\ref{sec:simulator_agent}.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{simulator_new.pdf}
\caption{Architecture Diagram of Simulator}
\label{fig:simulator}
\end{figure}

\subsubsection{Road Network Graph}
We construct a directed graph as the road network in the service area from Open Street Map data \cite{osm}, so that a trajectory of each dispatch movement can be generated. We removed road edges with types indicating only for pedestrians. The simulator first finds the closest road edges to the coordinates and then conducts an A* search for the shortest path between them.

\subsubsection{ETA Model}
A trained ETA (Estimated Time of Arrival) model is used to estimate trip time for every dispatch. We trained a multi layer perceptron using historical trip records in the service area in May 2016. The input feature vector consists of sine and cosine of day of week, sine and cosine of hour of the day, pickup latitude, pickup longitude, dropoff latitude, dropoff longitude and trip distance. Since the purpose of the estimator is to achieve a reasonably accurate estimation with short simulation time, we use a relatively small model, which consists of two hidden layers consisting 32 units following rectifier nonlinearity. We shuffle and split the trip records, preparing 70\% for training and 30 \% for validation. With the trained model, root-mean-square error (RMSE) for the training and validation datasets are 4.740 and 4.739 minutes respectively.

\subsubsection{Matching Algorithm}
We assign the closest available vehicle to each request. If there is no available vehicles in the range of five kilo-meters from the pickup location, the request is rejected. An assigned vehicle heads towards the pickup location with trip time predicted by the ETA model. After picking up passengers, the vehicle drives to the drop off location in the trip time on the actual trip record.

\subsection{Framework implementations}\label{sec:simulator_agent}

The agent in Figure~\ref{fig:simulator} runs either the RHC or DQN algorithm (Algorithms~\ref{alg:RHC} and~\ref{alg:DQN})). We detail our implementations of both in this section, after outlining the demand prediction that both algorithms use.

\begin{figure}[b]
\centering
\includegraphics[width=0.45\textwidth]{prediction}
\caption{Example of predicted demand heat map}
\label{fig:prediction}
\end{figure}

\subsubsection{Demand prediction}
To predict future demand, we build a small convolutional neural network. The output of the network is a $212 \times 219$ image in which each pixel stands for the predicted number of ride requests in a given region in the next 30 minutes. The network inputs six feature planes whose size is also $212 \times 219$: actual demand heat maps from the last two steps and constant planes with sine and cosine of day of week and hour of day. The first hidden layer convolves 16 filters of $5\times5$ with a rectifier nonlinearity. The second layers convolves 32 filters of $3\times3$ followed by a rectifier nonlinearity. The final layer convolves 1 filter of kernel size $1\times1$ again followed by rectifier nonlinearity. We preprocessed the dataset for creating heat map of demand distribution in each 30 minutes slot, splitting first 70\% for training and last 30 \% for validation without shuffling. We only consider cells with a passenger pickup in the past two timesteps. We predict that the demand in other cells is zeros. Root-mean-square errors (RMSE) for the training and validation datasets are 1.047 and 0.980 respectively. Figure ~\ref{fig:prediction} shows an example of target and prediction images.

\subsubsection{RHC Implementation}
Since the RHC optimization involves $M \times M \times T$ variables, the number of regions significantly affects the computational time. Thus, we use the taxi zones shown in Figure ~\ref{fig:demand} as our dispatch regions because the number of zones is only 226 but they still distinguish between regions with different taxi demand patterns. Predicted demand in each zone is calculated by aggregating outputs of the demand prediction model. The other key hyper parameters are the maximum lookahead time steps $T$ and cycle time $\Delta t$. We want $T \times \Delta t$ to be greater than 30 minutes and select $\Delta t = 15$ minutes and $T=3$. 

The destination distribution given origin, $P_t(d|o)$, was extracted from training data. We count the number of trips between taxi zones grouped by day of week and hour of day.

\subsubsection{DQN Implementation}
For the DQN policy, we use larger grid cells as dispatch regions because we can utilize spatial convolution. We divide the entire service area into $43\times 44$ grids each of which is around $800 \times 800$ m$^2$. The action space comprises a maximum of 7 moves in horizontal and vertical directions from the current cell, resulting in a $15 \times 15$ map for each cell. We select $\Delta t = 1$ minute and $T=30$.

% \subsubsection{Model Architecture}
Figure ~\ref{fig:network} presents the architecture of the Q-network. We use a convolutional neural network architecture in which there is a separate output unit for each possible action, and only the state representation is an input to the network. The outputs correspond to the estimated Q-values of the individual actions for the input state. The input to the network consists of a stack of heat maps ($23\times23\times12$) and auxiliary features ($15\times15\times12$). The first hidden layer convolves 16 filters of $5\times5$ with the only heat map features applied a rectifier nonlinearity. The second and third layers convolves 32 and 64 filters of $3\times3$ followed by a rectifier nonlinearity. The auxiliary input is applied 32 filters of $1\times1$ convolution with rectifier nonlinearity activation. Then, the two input branches are merged, following another convolutional layer ($128\times1\times1$). The final layer convolves 1 filter of kernel size $1\times1$.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{network}
\caption{Q-Network Architecture}
\label{fig:network}
\end{figure}

% \subsubsection{Features}
Table ~\ref{table:features} presents the input features for the network. Before putting demand and supply heat map images into the network, we crop and zero-pad the image according to each vehicle's position so that the vehicle's position becomes the center of $51\times51$ size images. Then, we apply different sizes of average pooling with stride (1, 1) to the shifted heat maps, resulting in $23\times23\times12$ feature maps. Auxiliary features are constructed from 12 features mapping to $15\times15$ plane.

\begin{table*}[t]
\caption{Input features for neural networks}
\label{table:features}
\begin{center}
\begin{tabular}{|l|l|c|c|l|} \hline
Type & Feature & Plan size & \# of planes & Description \\ \hline
Main & Demand & $51\times51$ & 1 & Predicted number of ride requests next 30 minutes in each region \\
 & Supply & $51\times51$ & 3 & Expected number of available vehicles in each region in 0, 15 and 30 minutes \\
 & Idle & $51\times51$ & 1 & Number of vehicles in $\mathcal{I}_t$ in each region \\ \hline
Main* & Cropped & $23\times23$ & 5 & Main features applied (23, 23) cropping\\
 & Average & $23\times23$ & 5 & Main features applied (15, 15) average pooling with (1, 1) stride \\
 & Double Average & $23\times23$ & 5 & Main features applied (30, 30) average pooling with (1, 1) stride \\ \hline

Auxiliary & Day of week & $15\times15$ & 2 & Constant planes filled with sin and cos of the day of week \\
 & Hour of day & $15\times15$ & 2 & Constant planes filled with sin and cos of the hour of day \\
 & Position & $15\times15$ & 1 & A constant plane filled with 0 except current position of the vehicle with 1\\
 & Coordinate & $15\times15$ & 2 & Constant planes filled with current normalized coordinates of the vehicle \\
 & Move Coordinate & $15\times15$ & 2 & Normalized coordinate at this point \\
 & Distance & $15\times15$ & 1 & Normalized distance to this point from the center\\
 & Sensibleness & $15\times15$ & 1 & Whether a move at this point is legal\\ \hline

\end{tabular}
\end{center}
\end{table*}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{input}
\caption{Examples of input features}
\label{fig:input}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{q_values}
\caption{Examples of output Q-values}
\label{fig:output}
\end{figure}

% \subsubsection{Training Details}
Reinforcement learning is known to be unstable when a nonlinear function approximator such as a neural network is used to represent the Q function. This instability is mainly due to correlations in the sequence of experiences and the correlation between the action-values $Q(s,a)$ and the target values $r+\gamma \max_{a'}Q(s',a')$. Thus, we use experience replay to remove correlations in the observation sequence and smooth over changes in the data distribution, by storing observed transitions and randomly samples from this memory bank to update the network~\cite{schaul2015prioritized}. Second, we used a target network that is the same as the online network except that its parameters are only periodically updated, thereby reducing correlations with the target. In addition, Double DQN algorithm is used to prevent Q-learning's overestimation \cite{DDQN}. In Double DQN algorithm, when we compute target value $r_t + \gamma \hat{Q}(\phi_{t+1},a^*_t;\theta ^-)$, the selection of the action, in the argmax, is due to the Q-network with parameters $\theta$.

We used the RMSProp algorithm for training with minibatches of size 64. The behavior policy during training was $\epsilon$-greedy with $\epsilon$ annealed linearly from 1.0 to 0.05 over the first 5000 steps, and fixed thereafter. One of the biggest challenges to apply DQN to our multi-agent system is that all vehicles execute a learned varying policy, thus changing the dynamics of the environment from the perspective of individual vehicles over time during training. This change in the dynamics requires change in the optimal policy. In order to mitigate the change of the environment, we introduce another parameter $\alpha$ as the probability to take an action in each time step and increase it linearly from 0.3 to 1.0 over first 5000 steps. Thus, only 30 \% of the vehicles move at the beginning, which is roughly the similar percentage of vehicles taking movement actions in the optimal policy. Thus, if the Q-network gets close to the optimal policy over time, the number of vehicles moving in each time step does not vary significantly. We trained for a total of 20,000 steps and used a replay memory of the 10,000 most recent transitions. As the temporal evolution of one index of learning illustrates in Figure ~\ref{fig:learning}, our method was able to train complex neural networks in a stable manner. Once the average max-Q-values reaches 100 at around 5000 steps, it starts decreasing because the environment has also changed by improvement in fleet behaviors. This means that competition for gaining customers between taxis increases over time, thus decreasing average return individual taxi can gain.

\begin{algorithm}
\small
\caption{double Q-learning with experience replay}\label{euclid}
Initialize replay memory $D$\;
Initialize Q-network $Q$ with random weights $\theta$\;
Initialize target Q-network $\hat{Q}$ with random weights $\theta^-$\;
\For{episode=1:EP}
{
Initialize the Simulator\;
\For{$t=1:T_{max}$}{
Execute the dispatch order in simulator and observe fleet state $F_t$, future demand $W_{t:t+T}$ and reward $r_t^{(n)} (n \in \mathcal{I}_{t-\delta})$\;
Preprocess $F_t$ and compute $X_{t:t+T}$\;
\For{$n \in \mathcal{I}_{t-\delta}$}
{
Create a feature vector $\phi_t^{(n)} = \phi(f_t^{(n)}, X_{t:t+T}, W_{t:t+T})$\;
Store transition ($\phi_{t-\delta}^{(n)}, a_{t-\delta}^{(n)}, r_t^{(n)}, \phi_{t}^{(n)}, \tau_t^{(n)}$) in $D$\;
}
Sample random minibatch of transitions ($\phi_j, a_j, r_j, \phi_{j+1}, \tau_{j+1}$) from $D$\;
Set $a^*_j = \argmax_{a'}Q(\phi_{j+1}, a'; \theta)$\;
Set $y_j = r_j + \gamma^{1+\tau_{j+1}} \hat{Q}(\phi_{j+1},a^*_j;\theta ^-)$\;
Perform a gradient descent step on $(y_j - Q(\phi_{j},a_j;\theta))^2$ with respect to $\theta$\;
Every C steps reset $\theta^- = \theta$\;

Select a set of available vehicles $\mathcal{I}_t$\;
\For{$n \in \mathcal{I}_t$}
{
Create a feature vector $\phi_t^{(n)} = \phi(f_t^{(n)}, X_{t:t+T}, W_{t:t+T})$\;
With probability $\epsilon$ select a random action $a_t^{(n)}$
otherwise select $a_t^{(n)} = \argmax_{a} Q(\phi_t^{(n)}, a; \theta)$\;
Select a destination region $i$ from action $a_t^{(n)}$\;
Select $d_{t}^{(n)} = \argmax_{l \in \mathcal{L}_i} \eta_t(l)$\;
Add ($n, d_{t}^{(n)}$) to the dispatch order\;
Update $X_{t:t+T}$ based on $a_t^{(n)}$\;
}
}
}
\end{algorithm}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{learning_curve.pdf}
\caption{Training curves tracking the agent's average loss and average predicted action-value}
\label{fig:learning}
\end{figure}


==> memo.tex <==



==> reference_TR.tex <==
\begin{thebibliography}{9}
\bibitem{RHC} F. Miao, S. Han, S. Lin, J. A. Stankovic, D. Zhang, S. Munir, H. Huang, T. He, and G. J. Pappas, “Taxi Dispatch With Real-Time Sensing Data in Metropolitan Areas: A Receding Horizon Control Approach,” IEEE Trans. Autom. Sci. Eng., vol. 13, no. 2, pp. 463–478, Apr. 2016.
%
\bibitem{laporte1992vehicle} G. Laporte, ``The vehicle routing problem: An overview of exact and approximate algorithms,'' European journal of operational research, vol. 59, no. 3, pp. 345--358, 1992.
%
\bibitem{golden1998impact} B. L. Golden, E. A. Wasil, J. P. Kelly, and I.-M. Chao, ``The impact of metaheuristics on solving the vehicle routing problem: algorithms, problem sets, and computational results,'' Fleet management and logistics, pp. 33--56, 1998.
%
\bibitem{cordeau1997tabu} J.-F. Cordeau, M. Gendreau, and G. Laporte, ``A tabu search heuristic for periodic and multi-depot vehicle routing problems,'' Networks, vol. 30, no. 2, pp. 105--119, 1997.
%
\bibitem{wait} Kiam Tian Seow, Nam Hai Dang, and Der-Horng Lee, “A Collaborative Multiagent Taxi-Dispatch System,” IEEE Trans. Autom. Sci. Eng., vol. 7, no. 3, pp. 607–616, Jul. 2010.
%
\bibitem{demand1} D. Zhang, T. He, S. Lin, S. Munir, and J. A. Stankovic, “Dmodel: Online Taxicab Demand Model from Big Sensor Data in a Roving Sensor Network,” in IEEE International Congress on Big Data, 2014, pp. 152–159.
%
\bibitem{demand2} B. Li, D. Zhang, L. Sun, C. Chen, S. Li, G. Qi, and Q. Yang, “Hunting or waiting? Discovering passenger-finding strategies from a large-scale real-world taxi dataset,” in the IEEE International Conference on Pervasive Computing and Communications Workshops, 2011, pp. 63–68.
%
\bibitem{miao2017data} F. Miao, S. Han, A. M. Hendawi, M. E. Khalefa, J. A. Stankovic, and G. J. Pappas, ``Data-driven distributionally robust vehicle balancing using dynamic region partitions,'' in Proc. of ACM ICCPS, pp. 261--271, 2017.
%
\bibitem{zheng2017online} H. Zheng and J. Wu, ``Online to Offline Business: Urban Taxi Dispatching with Passenger-Driver Matching Stability,'' in Proc. of IEEE ICDCS, 2017.
%
\bibitem{robotic} R. Zhang and M. Pavone, “Control of robotic mobility-on-demand systems: A queueing-theoretical perspective,” Int. J. Rob. Res., vol. 35, no. 1–3, pp. 186–203, Jan. 2016.
%
\bibitem{kaelbling1996reinforcement} L. P. Kaelbling, M. L. Littman, and A. W. Moore, "Reinforcement Learning: A Survey", Journal of Artificial Intelligence Research, vol. 4, pp. 237-285, 1996.
%
\bibitem{DQN} V. Mnih, K. Kavukcuoglu, D. Silver, A. A. Rusu, J. Veness, M. G. Bellemare, A. Graves, M. Riedmiller, A. K. Fidjeland, G. Ostrovski, S. Petersen, C. Beattie, A. Sadik, I. Antonoglou, H. King, D. Kumaran, D. Wierstra, S. Legg, and D. Hassabis, “Human-level control through deep reinforcement learning.,” Nature, vol. 518, no. 7540, pp. 529–33, Feb. 2015.
%
\bibitem{DL} Y. LeCun, Y. Bengio, and G. Hinton, “Deep learning.,” Nature, vol. 521, no. 7553, pp. 436–44, May 2015.
%
\bibitem{recommend1} J. W. Powell, Y. Huang, F. Bastani, and M. Ji, “Towards Reducing Taxicab Cruising Time Using Spatio-Temporal Profitability Maps,” Springer, Berlin, Heidelberg, 2011, pp. 242–260.
%
\bibitem{recommend2} M. Qu, H. Zhu, J. Liu, G. Liu, and H. Xiong, “A cost-effective recommender system for taxi drivers,” in Proc. of ACM KDD, 2014, pp. 45–54.
%
\bibitem{ziebart2008navigate} B. D. Ziebart, A. L. Maas, A. K. Dey, and J. A. Bagnell, ``Navigate like a cabbie: Probabilistic reasoning from observed context-aware behavior,'' in Proc. of ACM UbiComp, pp. 322--331, 2008.
%
\bibitem{data} New York City Taxi and Limousine Commission. \url{http://www.nyc.gov/html/tlc/html/about/trip_record_data.shtml}
%
\bibitem{osm} OpenStreetMap \url{https://www.openstreetmap.org}
%
\bibitem{tensor} TensorFlow \url{https://www.tensorflow.org/}
%
\bibitem{schaul2015prioritized} T. Schaul, J. Quan, I. Antonoglou, and D. Silver, ``Prioritized experience replay,'' arXiv preprint arXiv:1511.05952, 2015.
%
\bibitem{DDQN} H. van Hasselt, A. Guez, and D. Silver, “Deep Reinforcement Learning with Double Q-learning,” Sep. 2015.

\end{thebibliography}

==> results_TR.tex <==
For our evaluation, we use the trip records from Monday, 6/6/2016 to Sunday, 6/12/2016. We assume that a day starts at 4 a.m. and ends at 4 a.m. in the following day. For example, Monday is defined as 24 hours from 4 a.m. on Monday 6/6/2016 to 4 a.m. on Tuesday 6/7/2016. For each day, we conduct a dispatch simulation with 8000 taxi vehicles, whose initial locations are chosen from the pickup locations of the first 8000 ride requests in our data. We run the simulation for 30 minutes without dispatching to initialize the environment. For each day of the week, we calculate three metrics: the average reject rate, wait time, and idle cruising time. The average reject rate can be computed as the number of rejects divided by the number of total requests in each day. We define the idle cruising time as the total driving time without passengers divided by the number of accepted requests. We also track the total trip time with passengers for each vehicle and compute the utilization rate, or fraction of time for which a vehicle is serving customers.

\subsection{Performance Results}
\noindent We show the results of each policy before comparing them.

\begin{figure*}[t]
\centering
\begin{subfigure}{0.46\textwidth}
\includegraphics[width=\textwidth]{rhc_lambda.pdf}
\caption{Reject rate, wait time, and cruising time for the RHC policy.}
\label{fig:rhc_lambda}
\end{subfigure}
%
\begin{subfigure}{0.46\textwidth}
\includegraphics[width=\textwidth]{rhc_T.pdf}
\caption{$T$ dependency of Average score in RHC policy}
\label{fig:rhc_T}
\end{subfigure}
\begin{subfigure}{0.46\textwidth}
\includegraphics[width=\textwidth]{dqn_lambda.pdf}
\caption{Reject rate, wait time, and cruising time for the DQN policy.}
\label{fig:dqn_lambda}
\end{subfigure}
\caption{All three performance metrics improve as the reject penalty $\lambda$ increases in the (a,b) RHC and (b) DQN policies.}
\end{figure*}

\textbf{RHC Policy.} 
We conduct a simulation with the test dataset using the RHC policy and compute each metric's average value over a week. Figure~\ref{fig:rhc_lambda} shows the results with different reject penalties $\lambda$ from 0 to 40. While all three metrics improve as $\lambda$ increases from 10 to 20, they take nearly the same value when $\lambda \geq 20$. This result indicates that in practice, our three performance criteria do not conflict, which is surprising: we would expect the idle cruising time to increase as the reject rate decreases, due to vehicles traveling longer distances to pick up more passengers. The result suggests that most vehicles are close to passenger demand locations, yet many requests are not served quickly due to drivers not realizing this proximity, highlighting the need for optimized dispatch algorithms. The floor on the reject rate as $\lambda$ increases, however, indicates that some requests are simply too far from any idle vehicles; our constraint on idle cruising time in (\ref{eq:opt_RHC}) then prevents any vehicles from traveling to their locations.

We also investigate the importance of maximum horizon $T$. In Figure~\ref{fig:rhc_T}, we show that the performance does not change significantly with $T \geq 1$, indicating that there is limited value to coordinating vehicle locations too far into the future, perhaps due to limited ability to predict future demands.

\textbf{DQN Policy.} 
Similar to RHC, we evaluate our DQN policy by a simulation calculating each metric's average value over a week. Figure~\ref{fig:dqn_lambda} shows the results with different reject penalties $\lambda$ from 0 to 20. As seen in the figure, as $\lambda$ increases, the reject rate improves until it reaches around 10 while the idle cruising time increase modestly for $\lambda \geq 10$. As for the RHC policy, all metric values level off as $\lambda$ increases, indicating that there is a nonzero floor for the reject rate.

\textbf{Performance Comparison.}
%
\begin{figure}
\centering
\includegraphics[width=0.49\textwidth]{summary.pdf}
\caption{DQN consistently outperforms RHC over one week.}
\label{fig:summary}
\end{figure}
%
We compare both dispatch policies to a simulation without dispatch. We summarize the results of no dispatch (NO), DQN with $\lambda = 10$ (DQN), and RHC with $\lambda = 20$ (RHC) in Figure~\ref{fig:summary}. Our results indicate that DQN outperforms RHC, but both significantly outperform no dispatching, indicating the value of optimized dispatch algorithms. They also suggest that DQN's better adaptability compensates for RHC's better coordination between vehicles.

In every day of the week, the reject rate and wait time in the RHC and DQN policies are significantly reduced compared to no dispatching, while the idle cruising time per request stays almost the same. The reject rate and average wait time of the DQN policy are reduced by 76\% and 34\% respectively compared with results of no dispatch, and by 20\% and 12\% compared with the results of the RHC policy. The idle cruising time of the DQN policy increases by 1.3\% compared with the time of no dispatch, and by 4.0\% compared with the time of RHC. Figure~\ref{fig:tue} shows the reject rate, wait time, and idle cruising time with RHC and DQN dispatch and without dispatch on Tuesday. DQN dispatch consistently reduces the reject rate and wait time more than RHC; Figure~\ref{fig:sat} shows that this holds for Saturday as well.

Figure~\ref{fig:utilization} shows the mean and minimum of the utilization rate over 8000 vehicles. While the mean utilization rates for the two methods are almost the same, the minimum utilization rate with the DQN policy is much greater than with the RHC policy. This smaller variance may be due to the fact that the DQN policy learns the optimal policy for an individual vehicle, meaning every vehicles tries to take the best actions for themselves. On the other hand, the RHC policy aims to maximize the total reward, which allows agents to take actions not for themselves, but for the system as a whole. Thus, DQN allows for a ``more fair'' distribution of rewards across the different vehicles. % This result is surprising, as it indicates that vehicles are not hurt by uncoordinated competition with the DQN policy.

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Tuesday.pdf}
\caption{DQN consistently outperforms RHC on Tuesday.}
\label{fig:tue}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{saturday.pdf} 
\caption{Performance comparison on a Saturday.}
\label{fig:sat}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{utilization.pdf}
\caption{Utilization rates vs. time. DQN has higher minimum but comparable mean utilization rates compared to RHC.}
\label{fig:utilization}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{util_hist}
% \caption{Histogram of utilization rates.}
% \label{fig:util_hist}
% \end{figure}


\subsection{DQN Advantages}
Despite the fact that the DQN policy does not make decisions for idle vehicles in centralized coordinated manner, our results show that DQN's reject rate is lower than RHC's on every day of week. We conjecture that such good performance is achieved due to the fact that DQN dispatch decisions can be computed in a streaming manner by an individual vehicle, thus enabling much faster dispatch decisions that can adapt to the environment state: compared to the fast computation of a neural network forward pass, which takes less than a hundred milliseconds on CPU, solving a linear program with tens of thousands of variables in RHC policy is more expensive, taking from seconds to tens of seconds. 

In order to investigate the effect of the dispatch cycle, we simulate the DQN policy with the same dispatch cycle as the RHC policy. The results are plotted as DQN* in Figure~\ref{fig:summary}, showing that the reject rate is almost the same as RHC. DQN's faster on-demand dispatch thus helps the agent to adapt to disruptive environmental changes more quickly than RHC, at the expense of centralized cooperation. Even when DQN and RHC have the same dispatch cycles, DQN's lack of model constraints allows it to compensate for its lack of coordination and perform as well as RHC.

Obeying the DQN policy is more beneficial for drivers than RHC, as DQN predicts the best action for each individual vehicle given its current state. Although RHC's central coordination enables more efficient fleet management as a whole, it may not lead to drivers' executing their individually optimal actions. Thus, the DQN policy may be more realistic to implement in real-world applications. Indeed, ride-sharing platforms like Uber and Lyft take this uncoordinated approach, which may partially explain their success in improving passenger wait times compared to traditional taxi services.

Other potential advantages of a DQN approach include the fact that the same network architecture and input features can be used for different service areas and its forward computation time is independent of the number of dispatch regions, thus making it suitable for large-scale fleet management system. In addition, it can easily take other characteristics of a vehicle such as speed, capacity, a driver's rate into account to make decisions by adding relevant features to the network input. 

